KernelPack-JAX: a meshless differentiable GPU framework for node generation and forward and inverse PDE problems

We present KernelPack-JAX, a meshless, differentiable, GPU framework in JAX for solving forward and inverse PDE problems in domains whose boundaries, including internal obstacles, are given only by samples of their smooth pieces. Our node generator is based on a new stacked representation of piecewise-smooth boundaries, in which a parametric partition of unity of each smooth piece induces the supports of a curl-free implicit partition of unity of the whole boundary. This representation keeps the edges and corners of the boundary and classifies every point of space without a global fit. Boundary and interior nodes are then selected by a parallel greedy independent-set algorithm that reproduces sequential Poisson-disk sampling exactly. We discretize elliptic and parabolic problems with radial basis function-generated finite differences (RBF-FD) on stencils selected by a new visibility heuristic to avoid crossing the boundary, with ghost nodes for the boundary conditions. In addition, our framework exposes a GPU sparse direct solver to JAX as a differentiable linear solve, so that Jacobians of time-dependent problems cost a small multiple of a forward solve. We derive error estimates that separate consistency from stability and bound the parameter error by the forward error. We demonstrate high-order convergence for Darcy flow, reaction-diffusion, and advection-diffusion in 2D and 3D domains, including one with an internal obstacle, and show that the recovered parameters largely follow the forward errors. We also present timings for every stage.

==> forwardSolverConstruction.tex <==
\subsection{Forward solver construction}
This is probably where we explain the kernepack solver object, your custom matvec and the construction of a forward "object". 

==> gen_forward_timings.tex <==
\begin{table}
\centering
\caption{Wall-clock times in seconds on the finest clouds ($h=0.04$) on one NVIDIA RTX 5090. Setup is the assembly of all RBF-FD operators (for advection--diffusion including the hyperviscosity operator and the estimate of $\tau_a$); check is the Arnoldi test of Section~\ref{sec:forward_linear_algebra}; solve is the direct solve (Darcy) or the SBDF3 time integration, for one parameter family. All times include just-in-time compilation.}
\label{tab:forward_timings}
\begin{tabular}{llrrrrr}
\toprule
Geometry & $p$ & $N$ & Problem & Setup & Check & Solve\\
\midrule
H-channel & 2 & 1134 & Darcy & 2.3 & 0.7 & 0.1\\
H-channel & 2 & 1134 & reaction--diffusion & 3.8 & 0.7 & 0.1\\
H-channel & 2 & 1134 & advection--diffusion & 9.6 & 3.0 & 1.0\\
H-channel & 4 & 1134 & Darcy & 2.6 & 1.1 & 0.9\\
H-channel & 4 & 1134 & reaction--diffusion & 4.0 & 1.1 & 0.5\\
H-channel & 4 & 1134 & advection--diffusion & 7.8 & 3.3 & 1.5\\
H-channel & 6 & 1134 & Darcy & 3.1 & 1.1 & 1.2\\
H-channel & 6 & 1134 & reaction--diffusion & 4.3 & 1.1 & 1.6\\
H-channel & 6 & 1134 & advection--diffusion & 11.9 & 4.1 & 6.3\\
treasure chest & 2 & 25675 & Darcy & 38.0 & 3.3 & 17.8\\
treasure chest & 2 & 25675 & reaction--diffusion & 31.2 & 3.3 & 1.3\\
treasure chest & 2 & 25675 & advection--diffusion & 62.0 & 5.7 & 4.8\\
treasure chest & 4 & 25675 & Darcy & 46.5 & 3.7 & 11.3\\
treasure chest & 4 & 25675 & reaction--diffusion & 25.0 & 3.7 & 2.4\\
treasure chest & 4 & 25675 & advection--diffusion & 73.2 & 10.9 & 12.2\\
treasure chest & 6 & 25675 & Darcy & 111.9 & 4.6 & 29.0\\
treasure chest & 6 & 25675 & reaction--diffusion & 34.2 & 4.6 & 11.3\\
treasure chest & 6 & 25675 & advection--diffusion & 209.2 & 37.8 & 66.3\\
\bottomrule
\end{tabular}
\end{table}


==> inverseSolverConstruction.tex <==
\subsection{Inverse solver construction}
We probably want to move the implementation stuff in here, right Varun?


\subsubsection{Model picking}

==> overview.tex <==
\section{Review} Because KernelPack consists of an end-to-end framework we would like to briefly review the component parts and the math that underlies their behavior.

\subsection{Node generation}
\subsection{RBF-FD}
\label{sec:RBFFDmath}
Radial basis functions as approximations of differential operators have been used and studied for many years \cite{ PowellRestart1977} and their behaviors and strength are well understood \cite{Powell1987RadialBF}. We utilize the RBF-FD method discussed in [VARUN CITATION] which we will briefly explain.

For each node $x_i$ in the computational point cloud, the RBF-FD method
constructs a local stencil
\begin{equation}
    X_i = \{x_{i_1}, x_{i_2}, \ldots, x_{i_n}\},
\end{equation}
where the stencil points are typically chosen as the $n$ nearest neighbors of
$x_i$. The goal is to approximate a differential operator $\mathcal{L}$ at the
center point $x_i$ by a weighted sum over the stencil,
\begin{equation}
    \mathcal{L}u(x_i) \approx \sum_{j=1}^{n} w_{ij} u(x_{i_j}).
\end{equation}
The weights $w_{ij}$ are computed by enforcing exactness on a local RBF and
polynomial approximation space.

In this implementation, polyharmonic spline RBFs are used. For a stencil $X_i$,
define the pairwise distance matrix
\begin{equation}
    r_{jk} = \|x_{i_j} - x_{i_k}\|,
\end{equation}
and the RBF interpolation block
\begin{equation}
    A^{(i)}_{jk} = \phi(r_{jk}),
\end{equation}
where $\phi(r)$ is a polyharmonic spline, for example
\begin{equation}
    \phi(r) = r^m.
\end{equation}
Polynomial augmentation is included for stability and algebraic exactness. If
$\{p_\ell\}_{\ell=1}^{q}$ is the local polynomial basis, define
\begin{equation}
    P^{(i)}_{j\ell} = p_\ell(\widehat{x}_{i_j}),
\end{equation}
where the stencil coordinates are locally centered and scaled,
\begin{equation}
    \widehat{x}_{i_j}
    =
    \frac{x_{i_j} - \bar{x}_i}{h_i}.
\end{equation}
Here $\bar{x}_i$ is the stencil centroid and $h_i$ is a local stencil width. These polynomials can be of any family with the properties changing with regards to the family chosen. 

The augmented local RBF-FD system has the form
\begin{equation}
    \begin{bmatrix}
        A^{(i)} & P^{(i)} \\
        \left(P^{(i)}\right)^T & 0
    \end{bmatrix}
    \begin{bmatrix}
        w_i \\
        \lambda_i
    \end{bmatrix}
    =
    \begin{bmatrix}
        \mathcal{L}\phi(\|x_i - x_{i_1}\|) \\
        \vdots \\
        \mathcal{L}\phi(\|x_i - x_{i_n}\|) \\
        \mathcal{L}p_1(\widehat{x}_i) \\
        \vdots \\
        \mathcal{L}p_q(\widehat{x}_i)
    \end{bmatrix}.
\end{equation}
The first $n$ entries of the solution are the RBF-FD weights $w_i$. The
remaining entries $\lambda_i$ can be discarded.

For the Laplacian, the right-hand side contains
\begin{equation}
    \Delta \phi(\|x_i - x_{i_j}\|)
\end{equation}
and the corresponding polynomial Laplacians. For first derivatives, the
right-hand side instead contains
\begin{equation}
    \frac{\partial}{\partial x_k}\phi(\|x_i - x_{i_j}\|)
\end{equation}
and the matching polynomial derivatives. Boundary operators are handled
similarly, by combining normal derivative and Dirichlet contributions. For
example, a mixed boundary operator of the form
\begin{equation}
    \alpha \frac{\partial u}{\partial n} + \beta u
\end{equation}
uses the RBF right-hand side
\begin{equation}
    \alpha \, \nabla \phi(\|x_i - x_{i_j}\|)\cdot n_i
    +
    \beta \, \phi(\|x_i - x_{i_j}\|).
\end{equation}

By assembling the polyharmonic spline with higher and higher degree polynomials, the weight matrix can represent the operator $\mathcal{L}$ to arbitrarily high degree limited only by the size of the stencil. 

\subsection{Automatic differentiation}
Automatic differentiation (AD) has existed almost as long as modern computing \cite{wengertAutoDiff} and has been improved and iterated on for many years now. It provides a way to compute derivatives of numerical programs by systematically applying the chain rule to the elementary operations from which the program is built. Unlike numeric differentiation which relies on on perturbation it is analytically correct up to the bounds of the computational representation of the function. AD is also distinct from its cousin symbolic-differentiation because it does not rely on the rearrangement of algebraic operations represented by symbols into a closed form representation. This is all because a stack of operations to run can be treated as a composite function and thus the chain rule can be repeatedly applied to produce a partial derivative of the program. They are also typically more accurate than numerical-differentiation because they operate on the continuous version of a function and not its discrete representation.  

Two common modes are forward-mode and reverse-mode AD. Forward mode propagates directional derivatives alongside primal values and is often better for "tall" systems. Reverse mode propagates backwards using adjoints from output quantities and is instead better for "squat" systems.

For PDE-constrained problems, AD is useful because the map from parameters to observations is rarely a single closed-form formula. It may include geometry processing, assembly of discrete operators, linear or nonlinear solves, time integration, and loss evaluation. Provided these operations are expressed in differentiable array programs, AD can form gradients or Jacobians of the overall parameter-to-observation process. This enables inverse problems to be posed directly as optimization or root-finding problems over unknown coefficients, source terms, or model parameters.

There are, however, important practical distinctions between differentiating the mathematical solution operator and differentiating the particular algorithm used to compute it. For a linear solve
\begin{equation}
A(\theta) u(\theta) = b(\theta),
\end{equation}
the derivative of \(u\) is governed by the implicit relation
\begin{equation}
A(\theta)\,\frac{\partial u}{\partial \theta}
=
\frac{\partial b}{\partial \theta}
-
\frac{\partial A}{\partial \theta}u.
\end{equation}
Thus, an AD system may differentiate through a linear solve using an implicit rule rather than by differentiating every iteration of an iterative solver. This distinction is important in scientific computing, where direct, iterative, preconditioned, dense, and sparse solvers may all approximate the same discrete solution but expose very different computational traces to the AD system.

In practice, the efficiency and robustness of AD therefore depend not only on the mathematical problem, but also on the differentiable representation of the solver. Dense linear algebra routines, implicit differentiation rules, custom adjoints, checkpointing, and finite-difference or callback-based Jacobian approximations each represent different tradeoffs between memory use, compilation cost, accuracy, and implementation complexity. These considerations become especially important for time-dependent PDEs, where many solver applications may be composed before comparing a final or intermediate state to observations.



\subsection{Inverse problems}
\label{sec:inverseMath}
An inverse problem seeks to recover unknown quantities in a mathematical or physical model from indirect, incomplete, or noisy observations of the system. These unknowns may include initial conditions, material coefficients, source terms, boundary data, geometric parameters, or low-dimensional parameters defining a coefficient field. In contrast to a forward problem, where the governing equations and model inputs are used to predict the system state, an inverse problem uses observations of the state to infer the model inputs that most plausibly produced them. Inverse problems appear in many fields due to the importance of finding unknown information from limited observations. To illustrate consider the heat equation

\begin{equation}
\label{equ:ForwardHeat}
\frac{\partial u }{\partial t} = \alpha \nabla^2 u
\end{equation}

Now, let us imagine that the vector $\alpha$ varies with space like some arbitrary function $f(x,y)$. This function is unknown, but what is known is the forward progression in time of the process $u$. The goal of the inverse problem is to use information available to go backwards in time. This is difficult as for many problems there are a large number of different $f$ which may produce the same forward $u$. But in many cases there is enough information to, if not find the exact $f$, find a sufficiently close one.

In this paper we do this inversion via optimization using mathematical or physical models from observations of the system. Let \(\theta \in \mathbb{R}^p\) denote a finite-dimensional parameter vector and let \(F\) denote the forward map that sends parameters to observable solution values,

\begin{equation}
F : \mathbb{R}^p \to \mathbb{R}^m.
\label{eq:forward_parameter_map}
\end{equation}

Given observations \(u_{\mathrm{obs}} \in \mathbb{R}^m\), a common formulation is to define the residual

\begin{equation}
r(\theta) = F(\theta) - u_{\mathrm{obs}}.
\label{eq:inverse_residual_map_background}
\end{equation}

and seek parameters that minimize the mismatch between the predicted outcome and the correct outcome. The residual may also be interpreted as a root-finding problem for \(r(\theta)=0\). 

In order to perform optimization over this problem the process by which the forward answer is found must be differentiable. Without this it becomes extremely difficult to perform most robust optimization methods. Finding this derivative, especially for large complex functions, can be challenging. Consider that a function that has 100 timesteps would have a minimum of 100 nested functions each requiring the chain rule and it becomes impractical to perform this derivation by hand. Furthermore it is inconvenient to need to recalculate these derivatives every time the function changes. For this reason, we utilize automatic differentiation in order to create frameworks that can rapidly convert forward solves into inverse solves. 

Inversion does impose some limitations. First and foremost the cost of creating and storing gradients grows rapidly in both reverse and foward differentiation. Reverse-mode AD may require storing or reconstructing intermediate states from the forward computation, while forward-mode AD scales with the number of parameter directions being differentiated. For time-dependent PDEs, long time integrations can therefore increase memory use, compilation time, or recomputation cost unless the solver uses implicit differentiation, custom derivative rules, or a final-state-only objective. Furthermore the vector $\alpha$ contains less curvature information than the function $f$ that produced it, thus it creates a less meaningful optimization landscape. We remedy this with the use of parameterization. Instead of optimization equation \ref{equ:ForwardHeat} we instead optimize the following

\begin{equation}
\label{equ:forwardFunctionApprox}
\frac{\partial u }{\partial t} = \beta(p) \nabla^2 u,
\beta(p) \approx \alpha 
\end{equation}

Where $p$ is the parameters for the parameterized version of the PDE. Instead of optimizing for $\alpha$ we optimize over $p$. This not only decreases the size of the gradients (provided the size of the vector $p$ is less than the size of the vector $\alpha$) but also changes the differentiability of the function (provided $\beta$ is differentiable). This can be seen in the following example 

\begin{equation}
\label{equ:exampleDerivate1}
f(x) = \alpha \sin{(\pi x)}
\end{equation}

\begin{equation}
\label{equ:exampleDerivate2}
f'(x) = \pi \cos{(\pi x)}
\end{equation}

Whereas if we represent the vector $\alpha$ as a function $\beta(x) = \cos(x)$ we instead see

\begin{equation}
\label{equ:exampleDerivate3}
f'(x) = \pi \cos{(\pi x) - \sin(x)}
\end{equation}

which has a different minima. This does require the addition of a function $\beta$ which approximates the behavior of $\alpha$ which is, by the definition of an inverse problem, unknown. This is not as dire a strait as it seems though as there are several techniques available to find this function. Indeed, it is known that any function can be approximated via a sufficiently high degree polynomial \cite{polynomialApproximationTheory,Xun01092013}, meaning the difficulty lies in selecting and testing a large enough set of polynomials.



==> rbffd.tex <==
\section{Differentiable RBF-FD Solvers in JAX}
We really want to formulate everything to not only be GPU-parallelizable but inherently automatically differentiable and jittable. 

The construction of the RBF-FD solvers in JAX can, provided certain constraints are met, guarantee improved GPU usage and automatic-differentiation. As such both the construction of the RBF-FD weights and the usage of these weights is designed with those constraints in mind such that JAX can effectively parallelize the code and also calculate arbitrary derivatives for it. In this section we explain how the code is written in order to utilize JAX's strengths. 

\subsection{Parallel RBF-FD Weight Construction in JAX}

[SOMEWHERE IN HERE WE SHOULD INCLUDE CODE SNIPPETS]

In the RBF-FD assembly code, the computationally expensive part is the repeated construction and solution of many small local stencil systems. Each row of the global
finite-difference operator approximation matrix corresponds to one stencil center (Section~\ref{sec:forward_operators}), and each stencil requires a linear solve to acquire the weights for that node. Since these local calculations are independent they are embarrassingly parallel and thus a target for parallelization.

The implementation uses JAX to expose this independence to the compiler. Rather than constructing one stencil system, solving it, and then moving to the next stencil in a Python loop, the code collects all stencil point sets into one batched JAX array. The leading axis of this array indexes the stencil centers. Thus, one JAX array contains all local stencil geometries needed for the operator being assembled.

For RBF-FD weights, the main batched routines are JIT-compiled with \texttt{jax.jit}. For example, the code builds the batched pairwise distance matrices, polynomial augmentation blocks, RBF interpolation blocks, and operator right-hand sides inside compiled JAX functions. Once JIT-compiled, these array operations are lowered by XLA (Accelerated Linear Algebra\cite{}) into backend-specific kernels. On a GPU, this means the many independent stencil calculations can be executed in parallel rather than being driven one-by-one serial calls.

The core pattern is that a function is written to operate on an entire batch of stencils at once. For example, the input \texttt{x\_stencils} has a leading batch dimension, with shape similar to \texttt{(number\_of\_rows, stencil\_size, dimension)}. Operations such as pairwise distance construction use JAX broadcasting over this leading dimension. The resulting local matrices have shapes matching the size of the stencil and the size of the total domain. The call to \texttt{jnp.linalg.solve} is then also batched: JAX solves one local linear system per stencil center across the leading dimension. These vector operations are defined using JAX's \texttt{vmap} capabilities to convert single value functions into vector functions.

Conceptually, \texttt{vmap} is JAX's automatic way to turn a single-target functions into a batched function. If one wrote a function that computes RBF-FD weights for one stencil, \texttt{vmap} vectorizes that function so it applies independently to every stencil center. In this codebase, the RBF-FD fast path is mostly written with the batch dimension explicitly present in the arrays rather than as a direct \texttt{vmap} over a scalar stencil routine. This is the same parallelization idea: independent local stencil solves are represented as a single batched JAX computation. For example in the following simple Laplacian weight generation code.

\begin{lstlisting}[language=Python,label={code:weightGenerate}]
import jax
import jax.scipy as jsc
import jax.numpy as jnp

def getLapWStencil(cloud, stencil):
    LHS = jaxBuildLHS.buildLHSLap(cloud, stencil)
    RHS = jaxBuildRHS.buildRHSLap(cloud, stencil)

    LU = jsc.linalg.lu_factor(LHS)
    W = jsc.linalg.lu_solve(LU, jnp.transpose(RHS))[0:stencil.shape[0]].squeeze()

    Wrow = jnp.zeros((cloud.shape[0],))
    WfilledRow = Wrow.at[stencil].set(W)

    return WfilledRow

getLapW = jax.vmap(getLapWStencil, in_axes=(None, 0))
\end{lstlisting}

The code also uses \texttt{vmap} in nearby batched linear algebra utilities, for example when applying the same small operation across many local systems. The general pattern is:
\begin{itemize}
    \item use \texttt{vmap} when a per-stencil operation is easiest to express as a single-stencil function lifted over the stencil batch;
    \item use explicit leading batch dimensions when the whole calculation can be written naturally as batched array algebra;
    \item wrap the resulting batched computation in \texttt{jit} so XLA compiles it into efficient backend kernels.
\end{itemize}

This allows for the usage of \texttt{vmap} for applying the basis functions and polynomials. As well as the creation of the global matrix from local stencil calculations. 

[CODE SNIPPET OF RBF]

This has a very noticeable impact on speed. As does \texttt{jit}.

Without \texttt{jit}, JAX operations are still array operations, but Python does not guarantee asynchronous execution or full GPU utilization. When \texttt{jit} is used, the first time the function is called JAX traces the full batched weight-construction function, builds an XLA computation graph by reducing all vector operations down to pytree operations it can trace, and compiles the graph for the selected backend. This removes Python overhead from the inner assembly path and lets XLA fuse elementwise operations, schedule batched linear algebra, and place the computation on CPU or GPU as needed. It is important to stress that unlike other \texttt{jit} tools, JAX does not merely compile the python to bytecode but reduces the computation to operations on known primitives which, due to the static shape requirements, XLA can fuse and accelerate for GPU much more efficiently. 

After the batched RBF-FD weights are computed, the implementation scatters the local weights into the global operator matrix. This scatter step is also written with JAX array operations: row indices, column indices, and values are flattened from the batched stencil representation and inserted into the global operator. Thus, both the weight computation and the operator assembly avoid a stencil-by-stencil Python loop on the fast path.

In short, JAX parallelizes the RBF-FD assembly by representing all independent local stencil creation steps as batched computations. \texttt{vmap} provides the conceptual and practical mechanism for mapping single-variable logic across many vairables, while \texttt{jit} compiles the batched computation through XLA so the work can be scheduled efficiently on the available hardware without the need to write custom kernels or dispatch logic.

\subsection{Sparse Matrix Operations}
\label{sec:sparseMatOp}
Have to be custom to get past JAX's nascent inherent sparse matrix support if we want to stay automatically differentiable.

While JAX does provide an experimental sparse toolkit, it is currently unstable and no longer under active development. As such it was necessary to implement a custom sparse object and respective operations. This bespoke sparse array object underlies much of KernelPack and is based on the COO layout style. An array that is to be used for $Ax=b$ is represented as a shape vector, a vector containing the values and a vector containing the indices. This uses a custom matvec product and vecmat product. These are shown below

[CODE SNIPPETS]

By default, KernelPack assembles forward solver objects using these vectors, which decreases the memory footprint. Furthermore because they consist of a nested pytree, they are amenable to JAX's jitting and differentiation. One cost is that preconditioners that are designed either to work on JAX sparse objects or on dense matrices must be rewritten, but this also means that preconditioners can be designed to operate within the confines of differentiable programming. This is discussed more in section \ref{sec:precond}. 

This sparse representation is necessary in order to both improve scaling as larger matrices can be represented but also to improve speed as by avoiding explicit zeros the relevant data can be stored in more localized areas in memory. Possibly even entirely contiguously. In addition, operations can be performed directly on both the indices and the values in parallel and without copying the values elsewhere in memory.

\subsection{Differentiable Solver Design}
Mathematically, what does it take to make a solver differentiable?  Why do you need not just $A$ but $A^T$.

Finally, KernelPack-JAX is built to allow for fully differentiable solvers. At a high level this means is that all operations are built out of other operations which are themselves differentiable. This requirement does impose some restrictions, however the potential benefits are large.

First the foremost because automatic differentiation requires all component functions to be automatically differentiable, the solver in question should, ideally, avoid as much internal state logic as possible. This is because true/false based control flow is difficult to differentiate over, so methods that rely on checking things are runtime are hampered and should be avoided whenever possible. On the other hand loop based control with known bounds (e.g., \texttt{for $i$ in $n$}) are perfectly amenable to differentiation as they are treated as composite functions which allows for simple repeated application of the chain-rule.

Furthermore, in order to effectively differentiate a function one must have not only access to $A$ but also to $A^T$. This is because $A^T$ is needed to define the adjoint which allows for defining forward and reverse mode differentiation through the propagation of sensitivities in either direction. Having both forward and reverse mode differentiation means that problems that are many-input-to-few-outputs and few-inputs-to-many-output can both be cheaply handled without the need to use expensive finite differences or derivative collection. 

Furthermore, to effectively automatically differentiate composite functions is beneficial to have access to $A$ and also $A^T$ or an effective way of performing computations with this. This is because while forward-mode differentiation can be performed via a series of matrix-vector products, reverse-mode differentiation of the same system requires vector-matrix products due to the non-commutative nature of matrix multiplication. Thus in order to handle both many-inputs-to-few-outputs and few-outputs-to-many-inputs.

The obvious benefit of differentiability is the ability to generate arbitrary derivatives. This decrease development time substantially as unlike traditional solvers where Jacobian and Hessians must be hand-coded with KernelPack-JAX any function's Jacobian is automatically available by virtue of the function being in JAX. This also means that solvers can be written in a problem agnostic sense, simply taking the function to solve with as an argument. 

\subsubsection{JAX Custom linear solve}
Because KernelPack-JAX uses the custom sparse object discussed in section \ref{sec:sparseMatOp} several common solvers have been written to work with this sparse representation. These are implementations of well understood solvers such as GMRES \cite{classicGMRESpaper} but with the benefit of being built out of JAX differentiable primitives. New solvers can easily be added as well as long as they can be represented as matrix-vector operations. Any method that does not require the formation of the matrix or non-differentiable logic is appropriate. Of note is that while this is faster and less memory intensive, we provide several different automatic differentiation modes for this solver. This is because of tradeoffs between XLA graphs generated by the solver when it is treated differently. For example problems with a large number of iterations are ill-suited for direct representation as the repeated application of the chain rule causes the graph to increase in size rapidly so in those cases a surrogate system can be differentiated for better performance, or the derivative can be computed numerically. 

KernelPack also provides access to dense solver packages via a sparse-to-dense conversion. This means that libraries such as Lineax can be used should the available solvers be insufficient.

\subsubsection{Frozen Preconditioners}
\label{sec:precond}
Rejit if you don't.

Preconditioning is necessary for any problem involving sufficiently complex behaviors as ill-conditioning or size of the problem is liable to slow down performance or cause instability. However choosing a preconditioner, like choosing a solver, is a complex issue. Given the demands imposed by differentiability though, the preconditioners available to us are more limited. 

This is because preconditioners, in order to be effectively differentiable must be either very simple to extract (such as Jacobi preconditioning) or be calculated once and used repeatedly. This is because recalculation of many preconditioners, such as ILU, require either logic or a reconstruction of the linear solve. These either cause overhead due to repeated jitting every time the preconditioner changes or worse, a loss of differentiability. We therefore provide a few example preconditioners, such as jacobi preconditioning and frozen ILU.  Frozen in this case means that the ILU is made once at the beginning based on the initial guess and then is repeatedly used without being recomputed or at least having only minor changes made to it. Furthermore it is designed such that it is not considered inside the differentiation graph because otherwise the drop logic would cause the graph to become far more difficult to differentiate over.

\begin{lstlisting}[language=Python,label={code:preconditioner}]
...
applyMatrix=lax.stop_gradient(jnp.asarray(applyMatrix, dtype=float))
transposeApplyMatrix=lax.stop_gradient(jnp.asarray(transposeApplyMatrix, dtype=float))
...
\end{lstlisting}

In order to work alongside the custom linear solvers, this preconditioner is also defined in terms of matrix application and transposed matrix application instead of creating the dense matrix object.

% \section{Inverse Problems}
% \label{sec:inverProblemSetup}
% Having set up the forward solver like the geniuses we are, here's how you would generically solve inverse problems in JAX using optimization and rootfinding libraries. Code snippets, math if necessary. AT least call back to Section 2.4 as needed.

% Having created a forward solver context, it is trivial to create an inverse solver. As discussed in \ref{sec:inverseMath} the structure of an inverse problem in KernelPack is as a parameterized optimization problem with an objective function containing the forward equation. Provided one has the correct solution they want to invert towards and a parameterized forward equation the objective function can be as little as a function that runs the forward solve and compares against the true solution. Like so

% \begin{lstlisting}[language=Python,label={code:inverseProblemDefinition}]
% import lineax
% import optimistix as optx

% def objectiveFunction(params, args):
%     pred = runSystem(params) #the user defined forward solve
%     residual = trueSolution - pred

%     return residual


% linear_solver = lineax.AutoLinearSolver(well_posed=False)

% solver = optx.LevenbergMarquardt(
%     atol=1e-8,
%     rtol=1e-8,
%     linear_solver=linear_solver,
% )

% sol = optx.root_find(
%     objectiveFunction,
%     solver,
%     y0=paramsFirstGuess,
% )
% \end{lstlisting}

% Because this objective function is designed such that all it's components are differentiable, JAX can automatically compute it's gradient which means that optimization algorithms can be easily used. Furthermore because we can assume that there is a set of parameters for which the true solution is the result we can also safely use root-finding methods as the output of this optimization function will be zero ($\pm$ noise) at those parameters (\ref{eq:inverse_residual_map_background}). This is important because root-finding methods are typically faster to converge than optimization algorithms provided certain assurances about problem behavior \cite{rice1983numerical, albertoPaper}.

% This optimization loop does introduce some complexities however. For example it is possible for the optimizer to test parameters which can cause the forward solver to fail. For example consider a case in which the parameterized function contains $\frac{1}{x}$ in the forward solve. Should the optimization path decide to test $0$ the forward solver would fail as would the optimization loop due to the discontinuity. This can be remedied with the use of Optimistix's dense root-finding solvers. These solvers are able to adjust for ill-conditioned and ill-behaved optimization paths by switching to SVD or least-square methods if needed. These can work even in cases in which Krylov-methods fail. Increasing the accuracy of the forward solve can also remedy this as by moving towards the "true" solution of the forward equation it is less likely that impossible numbers will be tested [THIS SEEMS TO BE THE CASE, BUT I HAVE NO IDEA WHY. MAYBE BECAUSE AS h DECREASES SVD AND GMRES APPROCH THE SAME SOLUTION?]

%\subsubsection{Model selection}
%This is where we discuss our model/faimly pickers since %they're important for dealing with uncertainty


% \subsection{Fully Parallel Weight Creation}
% Because the weight for each point is independent of the weights for any other point, the problem of creating the system and solving for the weights at each point is embarrassingly parallel. Therefore it is natural to map the creation of the weights at a stencil onto parallel hardware such as a GPU and perform the mapped version over a collection of all the stencils at once. Such a method is effective at scale and only requires a small upfront cost in the form of KNN-tree creation.

% Because the stencils are all of the same size, they can be efficiently mapped onto a single set of instructions for weight creation, this allows for both simplified kernel writing, accelerated computation and consistency of order. 

% We utilize the RBFFD scheme used in \cite{Varun2020RBFFD} as while it is used in that paper for advection-diffusion it generalizes well to any process that can be represented as a combination of linear-operators. Because the method is discussed in great detail within \cite{Varun2020RBFFD} we will give only a brief overview. Each point in a point cloud has a weight computed via a linear system consisting of a radial-basis function and a polynomial basis evaluated at each point and its $K$ neighbors. Because both the radial-basis function and the polynomial basis are differentiable JAX is able to automatically produce the derivatives needed to create the right-hand-side for a linear system representing the application of a given linear operator on those points. Furthermore it also provides an equation for hyperviscosity which is needed as the gradient operator when represented via RBFFDs produces spurious Eigenvalues. 

% \subsection{Inverse problems}
% Having utilized JAX in order to generate the operator matrix, it becomes possible to create a fully differentiable solver for inverse problems. This requires little modification, but the benefits are great.

% Imagine the following problem, given a box containing fluid at some temperature and a final state for that box, find the diffusion coefficient. Several methods exist to do this, but most of them rely on either statistical models or apriori information about the system. However because the weights for this system were computed using our JAX-RBFFD the components, the functions to create said components and the forward solve are all fully differentiable the can be easily inverted by converting the problem to an optimization problem.

% To demonstrate: the previously mentioned example is presented.

% \begin{equation}
% \label{equ:diffusion}
% \frac{\partial u}{\partial t} = \alpha \Delta u
% \end{equation}

% If $\alpha$ is unknown, it can be very difficult to recover. However, the equation can be rewritten to produce an optimization problem who's solution is near the the correct $\alpha$. This just requires some simple rearranging.

% Given an initial state $u_0$, an end state $u_T$ and the matrix and vector objects required to transform one into the other, in this case a matrix $L$ representing the Laplacian operator, we can assume there is an $\alpha$ for which 
% \begin{equation}
% \label{equ:diffusionState}
% \alpha L u_0 - u_T = 0 
% \end{equation}

% This can further be rewritten as a function $g(\alpha')$ who's value is minimized at or near the true $\alpha$

% \begin{equation}
% \label{equ:diffusionalpha}
% g(\alpha') = \alpha' L u_0 - u_T
% \end{equation}

% To optimize this, first a forward solver is created that solves this diffusion problem in terms of $\alpha$, then this forward solver is used to define an objective function $O$ which is then optimized for. It is important that the forward solve is fully differentiable. In this paper lineax is used\cite{lineax2023} for differentiable linear solvers. The implementation of this is described in detail in \ref{code:forwardFunction}.

% By recasting the inverse problem as an optimization problem. The result of this optimization problem can take multiple form depending on the method used to find the unknown values.

% \subsubsection{Parameterization}
% Of important note is that because of ill-posedness of many inverse problems it quickly becomes impractical to learn the value of the full $\alpha$ directly. Instead it is better to define a forward solve in term of a parameterized model function with fewer parameters \cite{Xun01092013}. Not only does this decrease the computational load but it is also illustrative of the effects the parameters representing physical quantities have on the system. To illustrate this we will once again return to our fluid box example. 

% Let us say that our box is represented by a point cloud of $n$ points where $n$ is some large number. This means that the vector $\alpha$ must be of size $n$ and the Jacobian, residual and optimization landscape are of dimension $n$. This is prohibitively computationally expensive and consequently we advise the creation of one (or several) "model" functions $\mu$ which, given some parameters $\phi$, will create the full vector $\alpha$. Then optimize for the parameters of $\mu$. Methods for this are presented in the implementation section (\ref{sec:methods}).


% \subsection{Solver selection}
% Due to the large variety of problems that can be represented as inverse problems, no single ideal optimization algorithm exists. Therefore the choice of optimizer to use is problem dependent. Because of the use of JAX for the function creation, the user has access to arbitrary derivatives which allows a wide variety of algorithms. Picking an optimizer remains as much an art as a science though, and is outside the scope of this paper but many papers on the subject exist\cite{albertoPaper}. As a starting point Optimistix\cite{optimistix2024} has a large library of fully differentiable, JAX based optimization solvers. In this paper we utilized root-finding methods because the construction of the problem guarantees a root solution. That is to say because we are certain there is a value for which the objective function is 0 then using a root-finding method is preferable to using an optimization method, as they tend to converge faster. In the experiments presented in this paper we utilized Optimistix's root-finding algorithm, however versions using methods like ADAM are also viable.

% \subsection{Preconditioning} For complex problems, it may be that preconditioning is necessary for fast convergence of the forward solve. As a consequence there is a need for preconditioners that are amenable to automatic differentiation. This is harder than it may seem as many common preconditioning strategies are not currently supported by automatic-differentiation. Furthermore it is not guaranteed that \(\text{ILU}(\alpha'_{lower}L) = \alpha'_{lower}\text{ILU}(L)\) due to the nonlinearity of the ILU operation which means it cannot be easily precomputed. Thus because many ILU decomposition libraries rely on control flow which does not differentiate well, performing an ILU within the optimization loop is not preferable. This means that computing $M$ once and using it repeatedly for optimization iterations is ideal. A simple preconditioner $M$ that can be used is the creation of an ILU decomposition with a lower bound guess of $\alpha'$. This, while less than rigorous, does improve convergence. 

% \begin{equation}
% \label{equ:precondDef}
% M = \text{ILU}(\alpha'_{lower}L)
% \end{equation}

% The benefit of this method is that $M$ does not need to be recomputed during the optimization loop. 

% The diagonal of the A matrix can also be used, which can be found at each optimization step. As can any preconditioner method that can be described without control flow, keeping in mind that the addition of the computation of a preconditioner within the optimization loop increases the complexity of the objective function which increases the complexity of the optimization problem. 


% \subsection{Constraints and optimizations}

% By the nature of inverse problems, loose definitions of this objective function can lead optimizations to an incorrect value which nevertheless "solves" the optimization problem. The study of the construction of optimization problems is far-reaching and beyond the scope of this paper, but some common examples have been included for convenience and clarity.

% \subsubsection{Example 1: Steady states}

% Once again utilizing equation \ref{equ:diffusion}, if $\alpha = 1e-8$ for example, the steady state of of equation is that all points are at the same temperature at which point no more change occurs. In theory if the only data available is at the final time then the optimization may arrive at a much higher $\alpha$ as this will more quickly reach the steady state where it will remain for the rest of the runtime. This can be solved with the inclusion of more intermediate data within the objective function such as a midway timestep that is not yet reached the steady state. For example a snapshot halfway through the process $u_H$ would be included in the objective function like so.

% \begin{equation}
% \label{equ:mixedObj}
% g(\alpha') = (\alpha' L u_0 - u_T) + (\alpha' \frac{L}{2} u_0 - u_H)
% \end{equation}

% \subsubsection{Example 2: Maximum and minimums}

% If physical characteristics of the problem are known, those can be used to speed up convergence. Continuing with equation \ref{equ:diffusion} it is known that diffusion must be between 0 and 1. Thus maximum and minimums can be defined and the optimizer will converge faster and avoid producing physically impossible results.

% This can rapidly accelerate the convergence of these optimization methods, as many of them are quick to recapture the "shape" of the function, but struggle with the scaling. Adding a tight bound avoids this scaling problem.

% \section{Method Implementations}\label{sec:methods}

% \subsection{Parallel RBF-FD}
% In implementation, the fully parallel nature of the method is done by constructing all stencil left-hand-sides and right-hand-sides in batch form. Rather than looping over points one at a time, the coordinates of all stencil points are gathered into vectors and passed through the same sequence of operations. This allows the radial basis function evaluations, polynomial basis evaluations, and operator applications to be mapped over all stencils at once. JAX therefore views each stencil as an instance of the same small dense linear algebra problem, which can then be dispatched efficiently to accelerator hardware.

% Following the polyharmonic spline RBF-FD formulation of \cite{Varun2020RBFFD}, each stencil weight vector is obtained from a local augmented interpolation system of the form

% \begin{equation}
% \label{equ:weightMatrix}
% \begin{bmatrix}
% \Phi & P \\
% P^T & 0
% \end{bmatrix}
% \begin{bmatrix}
% w \\
% \lambda
% \end{bmatrix}
% =
% \begin{bmatrix}
% d \\
% q
% \end{bmatrix},
% \end{equation}

% where \(\Phi\) is the matrix of pairwise radial basis function evaluations over the stencil, \(P\) is the polynomial basis evaluated at the stencil nodes, $w$ is the vector of RBF-FD weights. The right-hand side terms $d$ and $q$ are constructed by applying the target differential operator to the radial basis function and polynomial basis respectively. After solving this augmented system, only the weights $w$ are retained for use in the discretized operator, while $\lambda$ is discarded.

% The RBFFD systems used in this paper are constructed using a polyharmonic spline radial basis function augmented by a polynomial basis. For two points $x$ and $x_c$, where $x_c$ is the center of the stencil and $x$ is all other points in the stencil, letting $r_c = \|x-x_c\|_2$, the radial part is taken to be
% \begin{equation}
% \label{equ:radialFunctionLHS}
% \phi(r_c) = r_c^m,
% \end{equation}
% where $m$ is an odd positive integer. In this work, the radial basis function is not used alone, but is augmented with a family of multivariate polynomials in order to guarantee polynomial reproduction and improve stability of the local approximation.

% Let $\{p_k(x)\}_{k=1}^Q$ denote a polynomial basis of total degree at most $\ell$. In two dimensions, this family includes terms such as
% \begin{equation}
% \label{equ:2dSeriesLHS}
% 1,\; x,\; y,\; x^2,\; xy,\; y^2,\; \dots
% \end{equation}
% and similarly in three dimensions includes
% \begin{equation}
% \label{equ:3dSeriesLHS}
% 1,\; x,\; y,\; z,\; x^2,\; xy,\; xz,\; y^2,\; yz,\; z^2,\; \dots
% \end{equation}
% up to the prescribed total degree. These polynomial terms are evaluated at the stencil nodes to form the matrix $P$ in the augmented local system. The benefits of different polynomial families (such as Legendre) is not discussed in this paper.

% The left-hand side of the local interpolation problem is therefore built from two components: the matrix $\Phi$, whose entries are pairwise evaluations of the radial basis function over the stencil, and the matrix $P$, whose entries are evaluations of the polynomial family at those same stencil nodes. The right-hand side is constructed by applying the desired differential operator $L$ to both families. In particular, the radial portion is given by
% \begin{equation}
% \label{equ:radialPortionRHS}
% d_c = L\phi(\|x-x_c\|_2),
% \end{equation}
% while the polynomial portion is given by
% \begin{equation}
% \label{equ:polynomialPortionRHS}
% q_k = Lp_k(x).
% \end{equation}
% Thus the same two approximation families used to build the interpolation system also determine the operator-dependent right-hand side used to recover the RBF-FD weights.


% Because both the basis evaluations and the operator applications are differentiable, the composition of these functions is also differentiable and jittable..This is important not only for efficient forward solves, but also for inverse-problem objectives in which model parameters appear in coefficient fields, forcing terms or boundary data.

% In addition this formulation naturally accommodates the construction of multiple operators on the same cloud. Once stencils have been identified, the same batched geometric data may be reused to construct any linear operator such as Laplacian, gradient and boundary operators of consistent order. This reduces repeated setup work and provides a uniform pathway for building the discrete objects needed by both forward and inverse simulations.

% \subsection{Inverse problem}

% At the implementation level, the inverse problem is constructed by wrapping the forward solver as a differentiable map from a parameter vector $\theta$ to a discrete state. Denoting this map by $F(\theta)$, the inverse solve is carried out by comparing the predicted state against a reference state $u^{obs}$ and using that comparison to define either a residual vector or a scalar objective.

% In code, this forward map may be represented schematically as follows.

% \begin{lstlisting}[caption={Forward function definition},label={code:forwardFunction},language=Python]
% import jax
% import jax.numpy as jnp
% import lineax as lx

% @jax.jit
% def forward(theta):
%     coeff = build_coefficient(theta, x)
%     A, b = assemble_system(coeff, operators, boundary_data)
%     sol = lx.linear_solve(
%         lx.MatrixLinearOperator(A),
%         b,
%         solver=lx.AutoLinearSolver(well_posed=False),
%     ).value
%     return sol
% \end{lstlisting}

% Once the forward map has been defined, the inverse problem is expressed in terms of it directly. For example, if $u^{obs}$ is a known reference state, then one may define the residual as in equation \ref{equ:diffusionalpha}
% \begin{lstlisting}[caption={Objective function definition},label={code:objectiveFunction},language=Python]
% def residual(theta):
%     return u_obs - forward(theta)

% def objective(theta):
%     r = u_obs - forward(theta)
%     return 0.5 * jnp.dot(r, r)
% \end{lstlisting}

% The choice between these two forms depends on the nonlinear solver being used. Residual vectors are natural for root-finding and nonlinear least-squares methods, while scalar objectives are natural for minimization methods. In either case, the same forward routine is reused.

% The important implementation detail is that $F(\theta)$ is assembled entirely from differentiable components. The discrete operators, parameterized coefficient functions, boundary terms, and linear solves are all written in a form compatible with automatic differentiation. As a result, derivatives with respect to $\theta$ can be obtained directly from the forward implementation without requiring a separate adjoint derivation.

% For steady problems, $F(\theta)$ consists of the assembly and solution of a single linear system. For transient problems, $F(\theta)$ includes the full time integration procedure, so that the dependence on $\theta$ propagates through each time step before the predicted state is compared with the observed data. Thus the implementation pattern remains the same across both problem classes: construct the forward map, evaluate the mismatch against the observed state, and pass the resulting residual or objective to the nonlinear solver. Using this objective function it can be passed into the optimizer of choice, in our case Optimistix




% \subsubsection{Multiple models}

% This section needs expansion


% Because the goal of inverse problems involves the recovery of unknown information from potentially incomplete data it is important to be able to compare several different possible explanations for correctness. As such we provide a few paradigms for testing different parameterizations for inverting these PDEs. Both of these offer benefits, and other systems for testing different models can also be designed.

% First we present the multi-model multi-shape system. This involves defining several different families of functions that each has a distinct shape, and we order the effectiveness of the models and then focus on only the most promising models. This is done via the creation of several optimization loop objects, these objects are each assembled as in \ref{code:objectiveFunction} 



% \section{Performance Breakdown}\label{sec:performance}
% The space, computation and time complexity of the methods described will be explained here. Because it is difficult to impossible to predict the amount of redundant work that is done much of the calculations here are illustrative, but not rigorous.

% In the following equations, the following variables will be used.

% $N = \text{Number of points in } d \text{ dimensions}$,
% $Q = \text{Number of polynomials}$,
% $S = \text{Stencil size}$,
% $V = \text{valid neighbors}$,
% $S << N$,
% $V << S$.

% \subsection{Computation}
% When using the overlapped version, substantially fewer left hand sides (LHS) need to be calculated. In the fully parallel version, each point requires the construction of its own $(Q+S)^2$ system. On the other hand the overlapped version only requires 1 LHS created for each subset of points defined as valid in a stencil. 

% The creation of the LHS, while performed using batch operations, still calls for the computation of a large number of polynomials and the application of a given operator to those polynomials.


% \subsection{Space}
% The space required for the computation of the weights for a single point $(Q+S)^2 + (Q+S)$ which, if we perform for each points results in a total space usage of $N*((Q+S)^2 + (Q+S))$. Thus, if we run this on the GPU there must be at least that much space on the GPU.

% The overlapped version however uses the following space for a single point $(Q+S)^2 + (Q+S)*V$ which is larger, however because there is a high chance that a given stencil will produce several valid weights. Because of this we instead have the following $N_{subset}((Q+S)^2 + (Q+S)*V)$. In a well behaved system, or for a large polynomial degree the number of points obtained by each system means that less space is needed.


% \subsection{Time}
% Time is 


==> shared_siam.tex <==
\usepackage{lineno}
\usepackage{amssymb,amsxtra,amsmath}
\usepackage{latexsym}
\usepackage{ifthen}
\usepackage{graphicx}
\usepackage{calc,fancyhdr}
\usepackage{indentfirst}
\usepackage{algorithm,algorithmicx}
\usepackage{algpseudocode}
\usepackage{color}
\usepackage{bigints}
\usepackage{subfig}
\usepackage{booktabs}
\usepackage{pdfpages}
\usepackage{Article}

\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\B}{\mathbb{B}}
\newcommand{\dx}[1]{\mathrm{d} #1}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\lstsize}{\scriptsize}

\newsiamremark{remark}{Remark}
\newsiamthm{assumption}{Assumption}

% Author formatting is provided by the SIAM class.

\newcommand{\TheTitle}{KernelPack-JAX: a meshless differentiable GPU framework for node generation and forward and inverse PDE problems}
\newcommand{\TheAuthors}{A. Cattaneo, M. K. Ballard, R. M. Kirby, G. B. Wright, and V. Shankar}

% Sets running headers as well as PDF title and authors
\headers{KernelPack-JAX}{\TheAuthors}

% TODO: SIAM asks for an email address in each author footnote, as (\email{...}).
\author{Alberto Cattaneo\thanks{Kahlert School of Computing, University of Utah, Salt Lake City, UT 84112, USA.}
\and M. Keith Ballard\thanks{Materials and Manufacturing Directorate, Composite Performance, Air Force Research Laboratory, Wright-Patterson AFB, OH 45324, USA.}
\and Robert M. Kirby\thanks{Scientific Computing and Imaging Institute, University of Utah, Salt Lake City, UT 84112, USA.}
\and Grady B. Wright\thanks{Department of Mathematics, Boise State University, Boise, ID, USA.}
\and Varun Shankar\footnotemark[2]}
% % Authors: full names plus addresses.
% \author{
%   Varun Shankar\thanks{School of Computing, University of Utah, Salt Lake City, UT USA
%     (\email{shankar@cs.utah.edu}, \url{http://www.cs.utah.edu/\string~shankar/}). Corresponding author.}
%   %\footnotemark[3]
% }

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Submitted to the editors \today.}}

